Reconstruction of continuum robots by marker-free shape registration of image data using a kinematic model

Continuum robots are slender, flexible manipulators that navigate confined, curved workspaces and are gaining traction in aerospace, inspection, automation, and minimally invasive medical applications. Predicting their shape from physics-based models alone remains challenging, making accurate measurement of the deformed backbone essential for model validation and reference-data acquisition. We present an optimization-based shape-registration algorithm that fits a parametric three-dimensional curve directly to image observations within a photogrammetric pipeline, targeting marker-free measurement rather than sensing under occlusion. By matching reconstruction points to robot pixels, the method requires no prior knowledge of the robot's location in each image. Across most configurations, the estimated backbone deviates from ground truth by less than 1 mm (0.67% of the robot's length). On real concentric-tube continuum robots, the reconstruction agrees with ten discrete manual photogrammetric measurements over 18 configurations, while replacing the manual procedure with an automated pipeline that runs in roughly 0.5 s per configuration.

==> inc/CTCR_model.tex <==
% !TeX spellcheck = en_US
% !TeX root = ..\main.tex

\section{Validation methodology \& CTCR-Model etc. \jm{Kapitel ist momentan Resterampe fällt komplett weg}}\jm{Nur zitieren und 2...3 Sätze zu Details des Rucker-Modells}

\jm{Vorschlag: \enquote{Data generation -- artificial images}: Beschreibung, wie man zu der Kanüle und den Daten kommt und stattdessen Rucker und die Implementierungen einfach nur zitieren ohne große Beschreibungen.}

In this paper, we concentrate on the shape registration of  concentric tube continuum robots (CTCRs). CTCRs, as a special class of continuum robots with potential for miniaturization, are well-suited for minimally invasive surgery. To generate real images of CTCRs, we constructed a photogrammetric measurement system with two strategically positioned cameras, as shown in \figref{fig:photogrammetry}.

\label{sec:model}
\begin{figure}[htb]
	\centering
	\fontsize{8}{0}\selectfont
	\def\svgwidth{0.45\textwidth}
	\input{figs/photogrammetry_system_sketch.pdf_tex}
	\hfill
	\includegraphics[width=0.4\linewidth]{photogrammetry_system_real.png}
	\caption{A photogrammetric measurement system estimates the 3D position of a point by computing the coordinate where corresponding light rays intersect. On the right, the photogrammetric system used in this work is shown. The cameras, well visible due to their red marking, point into the direction of the concentric tube continuum robot.}
	\label{fig:photogrammetry}
\end{figure}


\mkh{Brauchen wir für die künstlichen Bilder und die Motivation der Optimierungsbasierten Schätzung}


\cite{rucker2010basemodel}
%\begin{align}
%	\CM \qquad\quad & \nonumber\\
%	{\psi'}_i(s) &= u_{iz}(s),  \\
%	{u}'_{iz}(s) &= A_i \sum_{j \in T(s)}  E_j I_j (\boldu_{ixy}^{\star})^\top B_{\psi_{ij}}(s) \boldu_{jxy}^{\star}, \label{PPP_eq_4}\\
%	\boldu_{ixy}(s) &= \frac{1}{(EI)(s)}\sum_{j\in T(s)} C_{\psi_{ij}}(s)E_j I_j \boldu^{\star}_{jxy}\\
%	u_{iz}(\ell_i) &= 0, \label{PPP_eq_uz_end_point}\\
%	\psi_i(0) &= \alpha_i - \beta_i u_{iz}(0), \label{PPP_eq_psi_init}\\
%	{\p'}(s) &= \Rm(s)\bolde_3, \label{eq:CM_p}\\
%	{\Rm'}(s) &= \Rm(s)\hat{\boldu}_n(s), \label{eq:CM_R}\\
%	\p(0) &= \p^0 \in \R^3\label{eq:CM_p0}\\
%	\Rm(0) &= \Rm^0 \in \SO, \label{eq:CM_R0}
%\end{align}

\jm{$A_i$ undefined}

%\cite{till2020quaternion}
%\begin{align}
%	{\p'}(s) &= \frac{1}{\normexp{\q}}\begin{bmatrix} 
	%		2(q_2q_4+q_1q_3)\\
	%		2(q_3q_4-q_1q_2)\\
	%		1-2(q_2^2+q_3^2)
	%	\end{bmatrix}\\\
%	{\q'}(s) &= \frac{1}{2}\begin{bmatrix}
	%		0 & -u_x(s) & -u_y(s) & -u_z(s) \\
	%		u_x(s) & 0 & u_z(s) & -u_y(s) \\
	%		u_y(s) & -u_z(s) & 0 & u_x(s) \\
	%		u_z(s) & u_y(s) & -u_x(s) & 0 \\
	%	\end{bmatrix}\q\\
%	\p(0) &= \p^0 \in \R^3\label{eq:QM_p0}\\
%	\q(0) &= \q^0 \in \R^4\label{eq:QM_R0}
%\end{align}

To generate artificial images, we generate completely black images. After solving the boundary-value problem (BVP) describing the CTCR, the solution $p(s)$ is projected onto the image planes. The resulting image coordinates are rounded and the corresponding pixels are set to white. 
Application of dilation, a morphological operation with a disk of radius 15 as structuring element, to the binary image enlarges the white areas to give the cannula a visible volume in the images. The results are shown in Figure~\ref{fig:artif_img}.


%\begin{figure}
%	\centering
%	\input{figs/ctcr_sketch}
%	\label{fig:ctcr_sketch}
%\end{figure}

\mkh{Noch Rohfassung, nochmal genau schauen wohin wir damit wollen. Aktuell noch sehr wirr. Schieben der Teile in andere Abschnitte?}

==> inc/Pose_estimation_epipolar.tex <==
% !TeX spellcheck = en_US
% !TeX root = ..\main.tex

\section{Epipolar-geometry-based 3D shape estimation}
\zd{shape estimation, pose estimation, shape registration oder backbone sampling. eine einheitliche Benennung benötigt}
\label{sec:binocular}
Sampling the backbone through epipolar geometry is a fundamental method that has already been employed in marker-free 3D shape registration of continuum robots \cite{Gilbert2015, Diezinger2022, liang2021learning}. \jm{@ZH: besser mit der Einleitung verzahnen. Gehen alle zitierten Autoren genauso vor wie du oder machst du hier in Teilen etwas neues?} Initially, a skeletonization process is implemented to extract the robot's backbone from images. The subsequent step involves identifying corresponding 2D image points in multiple cameras making use of epipolar geometry. Finally, with a set of pixel coordinates for established point correspondences in two images, and knowledge of intrinsic and extrinsic parameters of cameras, the 3D coordinates of these points can be computed through triangulation.

\subsection{Finding the backbone in 2D images}
Skeletonization serves as a foundational step before the backbone sampling using epipolar lines. In this phase, we extract the backbone of the robot's images, representing its primary structural features. In \figref{fig:backbone_image}, in a real image captured by a camera, apart from the tubes constituting the CTCR, there are extraneous elements such as frames and the light source screen, which need to be removed from the image. Additionally the image may contain white noise and isolated points. To filter out these noises and smooth object contours, we can apply operations of erosion (which removes pixels on object boundaries in an image) followed by dilation (which adds pixels to the boundaries of objects). The \mcode{cv2.morphologyEx} function is a useful open-source tool for realizing these operations. After noise filtering, the \mcode{skimage.morphology} function is then used for skeletonization, reducing binary objects to 1-pixel wide representations. 
This way we can extract the central line of the robot, serving as the backbone. 

After skeletonization, it is essential to eliminate distortion using the distortion coefficient vector since the process of finding corresponding points via epipolar lines must be performed on undistorted images. We can, for example, apply \mcode{cv2.undistortPoints} function for distortion correction. \jm{So far, we have not written about camera parameter identification and optical distortions; we have to add that later in front of this chapter}. As the final step, the set of points constituting the backbone should be organized in order, from the starting point (where the continuum structure exits the base) to the end point (the tip of the robot). This ordering can be achieved using an algorithm that identifies the longest path in the backbone of a binary image. The approach involves constructing a directed graph of the backbone and then utilizing the \mcode{dag_longest_path} function from \mcode{networkx} to determine the longest path. 

\begin{figure}
	\centering
	\input{figs/backbone_image}
	\caption{The image is skeletonized to obtain the central line, which serves as the backbone. Subsequently, distortion is removed to prepare for the generation of epipolar lines. \mkh{Sieht aktuell so aus als würde das Entzerren Fehler erzeugen, aber tatsächlich ist das Bild ja falsch und die rote Linie korrekt.}}
	\label{fig:backbone_image}
\end{figure}

\subsection{Identification of corresponding points using Epipolar geometry}
In this section, we will provide an introduction to the basic principles of epipolar geometry and an automated identification process of corresponding points using this principle.
\figref{fig:epipolar_geometry} depicts two ideal pinhole cameras observing the same object space point $P$. Since the 3D line $\overline{O_L P}$ passes through the optical center of the lens $O_\mathrm{L}$, the corresponding epipolar line in the right image must pass through the epipole $e_\mathrm{R}$.  When a spatial point is projected onto the left image as $p_\mathrm{L}$, its corresponding projection point on the right image must lie on the epipolar line $l_\mathrm{R}$. So, to find the corresponding point, one can identify the intersection point of the image backbone with the epipolar line. The epipolar line can be represented by the linear equation ${a}{x}+{b}{y}={c}$, which is encoded by a 3-element vector $({a},{b},{c})$. $\boldsymbol{l} (\mathrm{a},\mathrm{b},\mathrm{c})$ can be computed through the fundamental matrix using the following expressions \cite{Hartley2004,forsyth2003cv}:
\begin{align*}
	\boldsymbol{l}_\mathrm{R} = \boldsymbol{F}\boldsymbol{x}_\mathrm{L} \quad or \quad \boldsymbol{l}_\mathrm{L} = \boldsymbol{F}^{\mathrm{T} } \boldsymbol{x}_\mathrm{R},
\end{align*}
where $\boldsymbol{x}_\mathrm{L}$ and $\boldsymbol{x}_\mathrm{R}$ are homogeneous normalized coordinates of $p_\mathrm{L}$ and $p_\mathrm{L}$, respectively, after undergoing undistortion. 
The fundamental matrix $\boldsymbol{F}$ is a 3x3 matrix that serves as the algebraic description of epipolar geometry and satisfies the condition
\begin{align*}
	{\boldsymbol{x}_\mathrm{R}} ^{\mathrm{T}} \boldsymbol{F}\boldsymbol{x}_\mathrm{L}=0
\end{align*}
for any pair of corresponding points $p_\mathrm{L}\leftrightarrow   p_\mathrm{R}$ in the two images. The fundamental matrix can be derived from the camera matrices based on the following formula \cite{forsyth2003cv}:
\begin{align*}
	\boldsymbol{F}={\boldsymbol{K}_\mathrm{R}}^ {-1}\boldsymbol{\varepsilon }{\boldsymbol{K}_\mathrm{L}}^ {\mathrm{T}}\ \ \mathrm{mit}\ \ \boldsymbol{\varepsilon }=\left [  \boldsymbol{t}_{\times } \right ]\boldsymbol{R} 
\end{align*}
where matrices $\boldsymbol{K}_\mathrm{L}$ and $\boldsymbol{K}_\mathrm{R}$ correspond to the intrinsic parameters of the two cameras (including focal length and optical center). The matrix $\boldsymbol{\varepsilon}$ is called the essential matrix and $\left [\boldsymbol{t}_{\times } \right ]$ denotes the skew-symmetric matrix such that  $\left [\boldsymbol{t}_{\times } \right ]\boldsymbol{R}=\boldsymbol{t}\times \boldsymbol{R}$ is the cross-product of the vectors $\boldsymbol{t}$ and $\boldsymbol{R}$. The rotation matrix $\boldsymbol{R}$ and translation vector $\boldsymbol{t}$ constitute the extrinsic parameters, representing the relative pose of the cameras in a common reference frame. 
\begin{figure}
	\centering
	\input{figs/epipolar_geometry}
	\caption{Epipolar geometry describes the relation between two resulting views of two pinhole cameras. The points $O_\mathrm{L}$ and $O_\mathrm{R}$ denote the optical center of each camera lens. $p_\mathrm{L}$ and $p_\mathrm{R}$ represent the projections of point $P$ onto the image planes. The points at which the optical centers of the camera lenses project onto the other camera's image plane are referred to as epipoles or epipolar points, and are denoted by $e_\mathrm{L}$ and $e_\mathrm{R}$. The red line $l_\mathrm{R}$ in the figure represents the epipolar line, also known as the projection line, corresponding to the point set, whose projections onto the left image are denoted as $p_\mathrm{L}$}
	\label{fig:epipolar_geometry}
\end{figure}

We developed an automated process for identifying corresponding 2D image points through the use of epipolar lines, incorporating an automatic scanning mechanism that eliminates the need for manual marking on a point in one image. We developed and validated our approach using artificial images, allowing for a comparison with ground truth data. The 3D backbone shape of the CTCR is derived from simulation results \mkh{das Kürzel ist hier noch nicht definiert}. Following this, we project the 3D backbone onto the camera planes. \zd{Details von virtuelle Abb. Generation in Kap.2?} \jm{Würde ich zustimmen}

As the points on the backbone in image have already been sorted along the path direction during the skeletonization, we can generate epipolar lines in the order along the direction of the backbone in left image and sequentially identify the intersections of their epipolar lines with the backbone in right image. For the intersection search, we define the pixel point closest to the epipolar line as the intersection point.

Sometimes an epipolar line can correspond to multiple intersections with the backbone as it is shown in \figref{fig:bin_img_sequence}. In this case, following rules should be adhered to ensure the correct search order for intersection points between the epipolar line and the backbone:

\begin{enumerate}
	\item Since epipolar lines are drawn at every small segment along the backbone in image 0, in image 1 the next intersection point should be adjacent to the previous intersection point.
	\item The direction from one intersection point to another should follow the positive tangent direction of the backbone to avoid the reversal of searching directions for the intersection points. 
\end{enumerate}

\begin{figure}
	\centering
	\input{figs/bin_img_sequence}
	\caption{The order of identifying corresponding points needs to follow the sequence along the backbone. The arrows indicate the searching order, when an epipolar line corresponds to multiple intersections.}
	\label{fig:bin_img_sequence}
\end{figure}


\subsection{Finding the 3D backbone through triangulation}
With the pixel coordinates of corresponding points in two images identified, namely $(u_\mathrm{L}, v_\mathrm{L})$ and $(u_\mathrm{R}, v_\mathrm{R})$, our goal is to triangulate and obtain the three-dimensional world coordinates $(X_\mathrm{w}, Y_\mathrm{w}, Z_\mathrm{w})$ in robot's coordinate system, where the starting point of the robot is defined as the origin, and the exit direction of the robot at start point is defined as the $z$-axis. The relationship between pixel coordinates and 3D world coordinates is defined as follows:

\begin{align*}
	\begin{bmatrix}
		u_\mathrm{L}\\
		v_\mathrm{L}
	\end{bmatrix}
	=\boldsymbol{K}_\mathrm{L}\left (\boldsymbol{R}_\mathrm{L} \begin{bmatrix}
		X_\mathrm{w}\\
		Y_\mathrm{w}\\
		Z_\mathrm{w}
	\end{bmatrix} +\boldsymbol{t}_\mathrm{L} \right ) /Z_\mathrm{cL} \quad \mathrm{and} \quad
	\begin{bmatrix}
		u_\mathrm{R}\\
		v_\mathrm{R}
	\end{bmatrix}
	=\boldsymbol{K}_\mathrm{R}\left (\boldsymbol{R}_\mathrm{R} \begin{bmatrix}
		X_\mathrm{w}\\
		Y_\mathrm{w}\\
		Z_\mathrm{w}
	\end{bmatrix} +\boldsymbol{t}_\mathrm{R} \right ) /Z_\mathrm{cR},
\end{align*}

where $Z_\mathrm{c}$ is the depth value of the point in the camera coordinate system. Given $(u_\mathrm{L},v_\mathrm{L})$ and $(u_\mathrm{R},v_\mathrm{R})$, we can use \mcode{cv2.triangulatePoints}, which employs methods based on solving nonlinear systems of equations through iterative optimization algorithms, to find the optimal solution for $(X_\mathrm{w},Y_\mathrm{w},Z_\mathrm{w})$.

\zd{Wird es hilfreich sein, eine Darstellungsabbildung von Backbones 3D-Koordinaten in Kap.2 zu zeigen}
We designate the found set of 3D coordinates of points on the backbone as $\boldsymbol{p}_\mathrm{B}$. In the physical model, the 3D coordinates of the backbone are typically defined as a function of the arc length: $\boldsymbol{p}_\mathrm{B}=\boldsymbol{p}_\mathrm{B}(\boldsymbol{s}_\mathrm{B})$. However, we cannot directly obtain the arc length $\boldsymbol{s}_\mathrm{B}[i]$ for each point $\boldsymbol{p}_\mathrm{B}[i]$ in the reconstructed curve through backbone sampling using epipolar geometry. As an approximation, we can only calculate the straight-line distance between each pair of adjacent sampling points and then accumulate these distances.

\subsection{Limitations}

Using epipolar lines generally enables the rapid \jm{Yes, but why?} identification of corresponding points in images. However, challenges may arise in certain scenarios, particularly at the bending points of the backbone, where the epipolar line approaches the tangent direction of the backbone, as illustrated in Figure \ref{fig:bin_img_error}. In these localized regions, multiple points on the backbone may align with the epipolar line, posing a challenge in precisely determining the corresponding points. This can lead to minor protrusions or discontinuities in the reconstructed curve corresponding to these regions.
\begin{figure}
	\centering
	\input{figs/bin_img_error}
	\caption{At the point where the epipolar line approaches the tangent direction of the backbone, the epipolar line approaches multiple points simultaneously, among which $ \mathrm{P} _{\mathrm{2a}} $, $ \mathrm{P} _{\mathrm{2b}} $, and $ \mathrm{P} _{\mathrm{2c}} $ are the three closest points with hardly any deviation from the epipolar line. There is ambiguity in identifying the most accurate corresponding point. }
	\label{fig:bin_img_error}
\end{figure}

When conducting backbone sampling on real images, the deviation between the actual backbone and the reconstructed curve is likely to be more significant. This disparity is often exacerbated by various sources of error, with one prominent factor being the inherent imprecision in camera calibration in real-world scenarios. Achieving a $100\%$ precise camera matrix is a challenging task, leading to non-negligible deviations in the computed epipolar lines. Apart from inaccuracies in camera calibration, other sources of error play a relatively minor role in contributing to the observed deviations. These include factors such as camera resolution, optical errors introduced by the lens, sensor noise, rounding of coordinate values, and so forth.  

In summary, the accuracy of backbone sampling using epipolar geometry in practical applications is constrained by the errors in the calibrated camera matrix \mkh{benötigt mMn eine Begründung warum die Fehler der Kamerakalibrierung größer als die der Skelettierung sind}. Moreover, deviations are typically larger at the point where the epipolar line approaches the tangent direction of the backbone. On the other hand, in the 3D shape estimation obtained through epipolar geometry, the direct inclusion of arc length information for each point is not present. \jm{Vielleicht eher für Conclusion-Kapitel?}

\jm{Vllt. noch zusätzlich \enquote{numerische} Ergebnisse oder Genauigkeitsabschätzungen oder Bilder oder so ähnlich?}


==> inc/Pose_estimation_optimization.tex <==
% !TeX spellcheck = en_US
% !TeX root = ..\main.tex

\section{Optimization-based 3D pose estimation}
\label{sec:optimal}
In the previous section, we showed how stereo vision of binary maps can be used to derive 3D information of points along the continuum robot's backbone.\ 
However, this method has limitations; specifically, it lacks the ability to precisely quantify and control the arc lengths of reconstructed points.\ 
Additionally, as we showed in section~\ref{sec:results_binocular}, this approach produces inaccurate results for robots bending parallel towards one of the camera's viewing ray -- the line from a 3D point to the camera's center.\
This section introduces a new technique inspired by the differentiable rendering approach by Lu et al. \cite{lu2023diffrendering} without the need of rendering a 3D object.\
The observed image content is matched with projections of a 3-dimensional \mkh{space?} curve, to the same image planes.
%This method optimizes the match between a parameterized 3-dimensional curve projected onto image planes and the corresponding observed image content.\
When taking images, 3D information is lost.
In our case, one critical information missing is to which arc-length of the continuum robot a pixel corresponds.
Due to this unknown correspondence, the value of a reconstruction at a specific arc-length cannot directly be matched to the correct image pixels. We alleviate this by incorporating an iterative closest point formulation that matches pixels with the closest reconstruction point.

\subsection{Problem formulation}
%Let 
%\begin{align*}
%	r:\ [0,L]\times\R^m &\rightarrow \R^3\\
%	(s,\theta) &\mapsto r(s;\theta)
%\end{align*}
%and
%\begin{align*}
%	b:\ [0,L] &\rightarrow \R^3\\ s&\mapsto b(s)
%\end{align*}
%be two curves parametrized in their respective arc length $s$, where $b$ can be seen as the backbone of the robot and $r$ is the corresponding reconstruction.\ 
%$r$ has the parameters $\theta$ that we want to optimize.\
%The optimization problem we aim to solve is
%\begin{align}
%	\min_\theta \ & \int_{0}^{L} \left(b(s) - r(s; \theta)\right)^2 ds,
%\end{align} 
%where $L$ is the known length of $b$.\ 
%Three problems occur, when applying this optimization problem to the CTCRs:
%First, we can only observe $C$ known projections $T_\gamma(b(s))$ of $b$, with
%\begin{align*}
%	T_\gamma:\ \R^3 &\rightarrow \R^2\\
%	 p &\mapsto T_\gamma(p) \\
%	\gamma \ &\in \{1, ..., C\}.
%\end{align*}\
%For brevity, we will set $\gamma$ to 1 and omit it, \mkh{the derived algorithms are not effected by this.}\ 
%Second, we only get $M$ discrete points at $T(b(\sbi)$, the pixels corresponding to the robot.\ 
%Third, as crucial 3D information is missing, we do not know the values of \sbi, thus rendering a cost function for matching $b$ and $r$ at corresponding arc lengths impossible.
%
%One class of algorithms that deal with this correspondence problem are iterative closest point algorithms, proposed by Besl and McKay \cite{besl1992icp}.\
%These assume that, of the $N$ points $r( \srj)$, the one that is closest to $b(\sbi)$ is used for correspondence in the matching.\ 
%It is easy to see, that does not always find the true correspondence as shown in Figure~\ref{fig:reconstruction_optimal}, but over iterations, this error can decrease and the algorithm can converge to the optimal solution, while finding the convergence.\ 
%
%\begin{figure}[htb]
%	\centering
%	\input{figs/reconstruction_optimal}
%	\caption{The cost function is computed as the sum of all reconstruction errors.\
%	The reconstruction error is the distance of each cannula pixel to the closest reconstruction pixel.\ 
%	Initial matching errors like in the initial guess decrease over the iteration steps, so that in the end the matching is ideal.}
%	\label{fig:reconstruction_optimal}
%\end{figure}
%
%With the distance measure for each pixel ($i$) to the corresponding reconstruction point of index~$j$
%\begin{align}
%	d_i(\theta, j) = \normexp{T(b(\sbi)) - T\left(r(s^r_j;\theta)\right)},\ j \in \{1,...,N\} \ \forall \ i\in \{1,...,M\}
%\end{align}
%and the cost function
%\begin{align}
%	J(\theta, \underbrace{j_1, j_2, ...}_{j_i}) = \sum_{i=1}^{M} d_i(\theta, j_i),
%\end{align}
%this renders the following bi-level optimization problem \mkh{Ich glaub ich tret mir hier mit der Notation auf die Füße. Ich wollte eine Abkürzung für $j_1, j_2, ...$ einführen... $\boldsymbol{j}^\star?$}
%\begin{align}
%	\min_\theta \ & J(\theta, j^\star_i)\\
%	\st \ & \jistar  = \argmin_{j} d_i(\theta, j), \ j\in\{1,...,N\}, \ \forall \ i\in \{1,...,M\}. \label{const:jstar}
%\end{align}\ 
%This bi-level optimization problem is hard to solve, especially since the cost function in the constraint is not differentiable.\
%Since equation \eqref{const:j_approx} is no longer dependant on $\theta$, the optimization problem \OP is now a normal curve fitting with (admittedly falsely) labelled data.\
%Still, after convergence, we can use the solution of \OP and reinitialize $\tilde{\theta}$ with it. 
%This gives the following recursive sequence
%\begin{align}
%	\tilde{\theta}\left[k+1\right] & = \argmin_\theta \ J(\theta, j^\star_i[k]) \label{eq:opt_simple}\\
%	\jistar[k] & = \argmin_{j}  d_i(\tilde{\theta}, j), \ j\in\{1,...,N\}, \ \forall \ i\in \{1,...,M\} \label{eq:opt_simple_constr}\\
%	\tilde{\theta}\left[0\right] & = \tilde{\theta}_0,
%\end{align}
%which we will call \textit{multi-step} formulation in the following.\

Let us define two curves parametrized by their respective arc lengths \( s \). The first, \( b(s) \), represents the actual backbone of the robot. The second, $r(s; \theta)$, is the reconstruction we aim to determine by optimizing for the decision variables \( \theta \), influencing the curve's shape.\ These curves are defined as:
\begin{align*}
	b:\ [0,L] &\rightarrow \R^3\\ 
	s&\mapsto b(s),
\end{align*}
and
\begin{align*}
	r:\ [0,L]\times\R^m &\rightarrow \R^3\\
	(s,\theta) &\mapsto r(s;\theta)
\end{align*}
where $L$ is the known length of the backbone.
The optimization problem we need to solve aims to minimize the difference between the actual backbone \( b(s) \) and the reconstructed curve \( r(s; \theta) \) over the length of the backbone. This is formulated as
\begin{align}
	\min_\theta \ & \int_{0}^{L} \normexp[p]{ b(s) - r(s; \theta)} \, ds.
\end{align}
The cost function evaluates the difference between both functions at corresponding arc lengths.
However, several challenges arise when applying this formulation to continuum robots:
\begin{enumerate}
	\item We observe the backbone \( b(s) \) through \( C \) known projections \( T_\gamma(b(s)) \), with the projection function \\ \( T_\gamma:\ \R^3 \rightarrow \R^2 \) mapping 3D points to their 2D image representations, where \( \gamma \in \{1, \ldots, C\} \).
	\item The robot projections \( T_\gamma \) are images, i.e.\ a finite number of discrete pixels. Thus, the \( M_\gamma \) observed pixels that correspond to the robot are denoted as \( T_\gamma(b(\sbi)) \), where $\sbi \in [0, L] \, \forall \, i\in \left\lbrace1, 2, \dots, M_\gamma\right\rbrace$ are unknown arc-length values.
	\item As the values of \( \sbi \) are unknown, it is impossible to match \( b \) and \( r \) directly at corresponding arc lengths.
\end{enumerate}
Let us define the following index sets %TODO: sets enthalten was?
%\begin{align*}
%	B_\gamma &= \left\lbrace T_\gamma(b(s)) \, \left| \, s \, \in \left\lbrace s^\mathrm{b}_1, s^\mathrm{b}_2, ..., s^\mathrm{b}_{M_\gamma} \right\rbrace \right. \right\rbrace \\ 
%	R_\gamma(\theta) &= \left\lbrace T_\gamma(r(s; \theta)) \, \left| \, s \, \in \, \left\lbrace s^\mathrm{r}_1, s^\mathrm{r}_2, ..., s^\mathrm{r}_{N_{_{}}} \right\rbrace \right. \right\rbrace,
%\end{align*}
\begin{align*}
	\setG &= \left\lbrace 1, 2, ..., C \right\rbrace\\
	\setI &=  \left\lbrace 1, 2, ..., M_\gamma \right\rbrace \\ 
	\setJ &= \left\lbrace 1, 2, ..., N \right\rbrace 
\end{align*}
containing the indices of the images, the indices of pixels corresponding to the robot per image, and the indices of the fixed reconstruction discretization points, respectively.
This gives the sets of robot and reconstruction image coordinates 
\begin{align*}
	B_\gamma &= \left\lbrace \bgi = T_\gamma(b(\sbi)) \, \left| \, i \, \in \setI \right. \right\rbrace \\ 
	R_\gamma(\theta) &= \left\lbrace \ngj = T_\gamma(r(\srj; \theta)) \, \left| \, j \, \in \, \setJ \right. \right\rbrace,
\end{align*}
where $\left\lbrace s^\mathrm{r}_1, s^\mathrm{r}_2, \dots, s^\mathrm{r}_N\right\rbrace$ is the set of $N$ fixed arc-lengths at which $r$ is evaluated.
To address the previously mentioned challenges, we consider the iterative closest point (ICP) approach by Besl and McKay \cite{besl1992icp} as a basis for finding the optimal correspondence between the finitely many oberservations in $B_\gamma$ and \( R_\gamma \). ICP algorithms were first discussed for finding rigid transformations of a point cloud \( B \) to match it with a second point cloud \( R \), by minimizing the sum of distances from all points of  \( R \) to the closest point in \( B \), respectively. Unlike the seminal work, other authors suggested to use not only the \( R \)-to-\( B \)- but also the \( B \)-to-\( R \)-correspondences, see for example \cite{godin1994invcorrespondence}, as this can positively influence the convergence. Our approach assumes that the point in \( r( \srj) \) closest to a point on \( b(\sbi) \) should be used for matching in each iteration, which corresponds solely to the \( B \)-to-\( R \)-correspondence, since this yields less local minima. Even though this crude matching does not guarantee exact correspondence initially, iterative refinement can lead to an optimal solution as sketched in Figure~\ref{fig:reconstruction_optimal}.
\mkh{Erklärung Least Squares?}
% Figure warum B->R gut und R->B schlecht z.b. über Aufwickeln. und aktuelle fig. 5 später? Nach (17)?

\begin{figure}[htb]
	\centering
	\input{figs/reconstruction_optimal}
	\caption{Matching to circular arcs of the same length with $\theta$ as the radius. The cost function is computed as the sum of all reconstruction errors.\
	The reconstruction error is the distance of each cannula pixel to the closest reconstruction pixel.\ 
	Initial matching errors like in the initial guess decrease over the iteration steps, so that in the end the matching is ideal.}
	\label{fig:reconstruction_optimal}
\end{figure}

For the \( i \)-th pixel coordinates \bgi in image $\gamma$, the distance to the  \( j \)-th reconstruction point is given by
\begin{align}
	\dgi(\theta, j, i) = \left\|\bgi - \ngj\right\|_p^p, \ \bgi \in B_\gamma, \ \ngj \in R_\gamma(\theta).
\end{align}
\mkh{Kann man die Mengen so angeben? Sonst fehlt explizite Abhängigkeit von $\theta$...}
%\begin{align}
%	d_i(\theta, j) = \left\|T(b(\sbi)) - T(r(s^\mathrm{r}_j;\theta))\right\|_p^p,\ j \in \{1,\ldots,N\}, \ \forall \ i\in \{1,\ldots,M\}.
%\end{align}
%\begin{align}
%	d_\gamma(\beta, \nu, \theta) = \left\|\beta - \nu \right\|_p^p,\ \beta \in B_\gamma, \ \forall \ \nu\in R_\gamma(\theta), \ \gamma \in \{1, ..., C\}.
%\end{align}
The cost function to minimize is
\begin{align}
	J(\theta) = \sum_{\gamma\in\setG}\sum_{i\in\setI}\sum_{j\in\setJ} \dgi(\theta, j, i)\indg(\theta,j,i),
\end{align}
where the indicator function can be used for selecting certain elements from the sum.
In our case, as we interested in assigning the \emph{closest} point from $R$ to each pixel in $B$, the indicator function
\begin{align}
	\indg(\theta,j,i) = \begin{cases} 
		1, & j = \argmin\limits_{\tilde{j}} \dgi(\theta, \tilde{j}, i), \ \tilde{j}\in\setJ, \\
		0, & \text{otherwise}
	\end{cases}
\end{align}
is only 1 if the selected $j$-th reconstruction point minimizes the distance to the $i$-th pixel of image $\gamma$.
%\begin{align}
%	\setJ_\gamma^\star(\theta) = \left\lbrace \argmin_{j}  \dgi(\theta, j, i) \ | \ \forall \ i \in \setI \right\rbrace
%\end{align}
%\mkh{Ist das noch bi-level?}
This problem is challenging due to the non-differentiability of the indicator function. To simplify, we replace \( \theta \) with a current estimate \( \tilde{\theta} \) in the indicator function, yielding
\begin{align}
	\OP\qquad\ \nonumber\\
	\min_\theta \ & \bar J(\theta,\tilde\theta) = \sum_{\gamma\in\setG}\sum_{i\in\setI}\sum_{j\in\setJ} \dgi(\theta, j, i)\indg(\tilde\theta,j,i). \label{eq:cost_j_approx}
\end{align}
Since the indicator function is no longer dependent on $\theta$, the optimization problem \OP is now a normal curve fitting with between the \bgi and the closest \ngj, which (most likely) does not match points of corresponding arc-length.\
Still, after convergence, we can use the solution of \OP and reinitialize $\tilde{\theta}$ with it, meaning that you can alternate between solving \eqref{eq:cost_j_approx} and fixing $\tilde\theta$.
This gives the following recursive sequence
\begin{align}
	\tilde{\theta}\left[k+1\right] & = \argmin_\theta \bar J(\theta,\tilde\theta[k]) \label{eq:opt_simple}\\
	\tilde{\theta}\left[0\right] & = \tilde{\theta}_0,
\end{align}
which we will call \textit{multi-step} formulation in the following.\
%In \cite{besl1992icp}, convergence of the ICP algorithm is argumented for the least-squares registration of point clouds for rotations and translations, but the same arguments hold for non-linear functions, like $r$, and using more general optimization algorithms.\
%Assume all convergence assumptions for the non-linear curve-fitting problem \eqref{eq:opt_simple} are fulfilled, so \eqref{eq:opt_simple} will not increase the cost.\ 
%The resulting solution $\theta^\star$ is a local minimizer for fixed $\jistar[k]$.\
%In the next iteration, $\jistar$ is computed again.\
%For fixed $\theta$, $d_i$ can be easily minimized by brute-forcing all comparisons between the projected reconstruction points and $T(b(\sbi))$.\
%Since all $d_i(\theta, \jistar)$ are independent w.r.t. their corresponding $\jistar$, it is easy to see that for fixed $\theta$, any change to $d_i(\theta, j_i)$ will change $J$ accordingly.\ \mkh{Was ich sagen möchte ist das Folgende: Wenn sich ein $\jistar$ ändert, ändert das $d_i$ und die gleiche Änderung erfährt $J$, ohne dass sich der Wert eines der anderen $d_i$ ändert. Also reicht es zu zeigen, dass sich jedes d nicht verschlechtert.}
%
%\begin{theorem}[Convergence of the ICP optimization]
%	The ICP curve-fitting algorithm has the same convergence conditions as the algorithm for solving the curve-fitting problem \eqref{eq:opt_simple}.
%\end{theorem}
%\begin{proof}
%	%	Assume, the conditions for finding local minima of \eqref{eq:opt_simple} are met.\ 
%	%	Then at step $k$, the solution $\theta[k]$ is its local minimizer.\ 
%	The cost function $J(\theta[k], \jistar[k]) = \sum_{i=0}^{M} d_i(\theta[k], \jistar[k])$ is a sum of distances $d_i(\theta[k], \jistar[k])$.
%	Minimizing $d_i(\theta[k], j_i)$ w.r.t. $j_i$ results in the minimizer index $\jistar[k]$.\ 
%	If $\jistar[k+1] = \jistar[k]$, then $$d_i(\theta[k], \jistar[k+1]) = d_i(\theta[k], \jistar[k]).$$\
%	If $\jistar[k+1] \neq \jistar[k]$, then  $$d_i(\theta[k], \jistar[k+1]) \le d_i(\theta[k], \jistar[k]),$$ as otherwise $\jistar[k+1]$ would not be a minimizer of $d_i(\theta[k], j_i)$.\ 
%	That means that $$\sum_{i=1}^M d_i(\theta[k], \jistar[k+1]) \le \sum_{i=1}^M d_i(\theta[k], \jistar[k])=J(\theta[k], \jistar[k]),$$ which is the cost of the initial guess for \eqref{eq:opt_simple} at time step $k+1$. This shows that reassigning the point correspondences cannot increase the cost function, thus leading to a convergence of the non-negative cost function $J$, as long as the algorithm for solving \eqref{eq:opt_simple} does not increase the cost function.\
%\end{proof}\
%
%This idea can be extended to other series definitions, as this algorithm will converge as long as in equation \eqref{eq:opt_simple}, the cost does not increase.\ 
%This is useful, because if we solve \eqref{eq:opt_simple} until convergence, we probably missed the point, where we could have exchanged $\jistar$, due to another reconstruction point being closer.\ 
%Instead, we could also just apply one gradient descent step, giving the \textit{one-step} formulation
%\begin{align}
%	\tilde{\theta}\left[k+1\right] & = \tilde{\theta}\left[k\right] - \alpha\left.\frac{dJ(\theta, \jistar[k])}{d\theta}\right|_{\theta=\tilde{\theta}[k]}\\
%	\jistar[k] & = \argmin_{j} \normexp{T(g(\sbi)) - T(f(s^f_j;\tilde{\theta}\left[k\right]))}, \ j\in\{1,...,N\}, \ \forall \ i\in \{1,...,M\} \\
%	\tilde{\theta}\left[0\right] & = \tilde{\theta}_0,
%\end{align}
%where the correspondences are recomputed after each gradient-descent step.\ 
%In this case, using the Armijo condition of sufficient decrease would be a valid condition for guaranteeing convergence.

Besl and McKay \cite{besl1992icp} discuss the convergence of the ICP algorithm for least-squares registration of point clouds under rotations and translations.\
Their arguments can be extended to non-linear functions like \( r(s; \theta) \), adapting the methodology for more general optimization scenarios.\
Assuming all convergence criteria for the non-linear curve-fitting problem \eqref{eq:opt_simple} are met, we can ensure that the optimization of \eqref{eq:opt_simple} does not increase the cost function. Consequently, the solution \( \theta[k+1] \) obtained at each iteration forms a local minimizer for $\bar J(\theta,\tilde\theta[k])$, given the fixed indicator function.

In the subsequent iteration, \( \tilde\theta[k+1] \) is not necessarily the local minimizer of $\bar J(\theta,\tilde\theta[k+1])$, but it is straight-forward to show that the cost function does not deteriorate, as long as the algorithm for solving \eqref{eq:opt_simple} does not increase it.\ 
%With \( \tilde{\theta}[k] \) being constant, the minimization of \( d_i \) for each pixel can be achieved by exhaustively comparing all projected reconstruction points with their counterparts in \( T(b(\sbi)) \).\ 
%The independence of each \( d_i(\theta, \jistar) \) regarding their corresponding \( \jistar \) implies that changes in \( \jistar \) directly influence the cost function \( J \) without affecting the values of other \( d_i \) terms. 

\begin{theorem}[Convergence of the ICP Optimization]
	The ICP curve-fitting approach for our problem setting converges under the same conditions as those stipulated for solving the curve-fitting problem \eqref{eq:opt_simple}.
\end{theorem}
\begin{proof}
	The cost function $\bar J$ is the sum of distances between 
	Therefore, \( \sum_{i=1}^M d_i(\theta[k], \jistar[k+1]) \leq J(\theta[k], \jistar[k]) \), ensuring that updating the correspondences does not increase the overall cost function.\ 
	This non-increase in the cost function leads to the convergence of the algorithm, as long as the cost of \eqref{eq:opt_simple} does not increase.
\end{proof}

Extending this idea to other series formulations, we note that the algorithm converges as long as the cost in \eqref{eq:opt_simple} does not increase.\ 
This observation is crucial, especially when considering that solving \eqref{eq:opt_simple} to full convergence might overlook the ideal point to swap \( \jistar \) due to another reconstruction point becoming closer.\ 
An even simpler approach is to apply a single gradient descent step per iteration, leading to the \textit{one-step} formulation
\begin{align*}
	\tilde{\theta}[k+1] & = \tilde{\theta}[k] - \alpha \left. \frac{\partial \bar J(\theta, \tilde\theta[k])}{\partial \theta} \right|_{\theta = \tilde{\theta}[k]} \\
	\tilde{\theta}[0] & = \tilde{\theta}_0,
\end{align*}
Applying the Armijo condition here ensures sufficient decrease at each step, thereby guaranteeing convergence of this iterative process.\


\subsection{Section ist WIP -- Using the binocular vision for warmstarting}
\mkh{Diese subsection war vorher 6.3}
%Gradient-descent methods are designed to converge to local optima from an initial guess.\ 
%With the results from the binocular vision approach, estimates for backbone positions $\pb[i]$ and their corresponding arc-lengths 
%\begin{align*}
%\sB[i] &= \sB[i-1] + \norm{\pb[i] - \pb[i-1]} \ \forall i\in [1, N]\\
%\sB[0] &= 0\\
%\pb[0] &= \begin{bmatrix}
	%	0 & 0 & 0
	%\end{bmatrix}^T
	%\end{align*}
	%\mkh{Die Approximierung der s[i] passt vmtl. besser in Section~\ref{sec:binocular}.}
	%can be used for setting up an initial guess 
	%\begin{align}
	%\tilde{\theta}_0 = \argmin_\theta \sum_{i=1}^N \normexp{p[i] - r(s[i];\theta)}
	%\end{align}
	%by solving the non-linear least squares problem with known correspondences.\
	
	Gradient descent methods inherently converge to local optima. Depending on the initial starting point, this local optimum can be vastly different in quality.\ 
	In the context of our optimization algorithm, an informed and accurate initial guess can significantly accelerate the convergence process and enhance the quality of the solution. \
	\mkh{$p_B$ sollte in Section~\ref{sec:binocular} eingeführt werden.}
	Leveraging the results from our binocular vision approach, we obtain preliminary estimates for the backbone positions \( \pb[i] \) and their corresponding arc-lengths.\
	The arc-lengths are estimated as
	\begin{align*}
		\sB[i] &= \sB[i-1] + \norm{\pb[i] - \pb[i-1]} \ \forall i \ \in \{1, ... N\},\\
		\sB[0] &= 0,\\
		\pb[0] &= \begin{bmatrix}
			0 & 0 & 0
		\end{bmatrix}^T.
	\end{align*}
	
	Utilizing these estimates, we construct an initial guess
	\begin{align}
		\tilde{\theta}_0 = \argmin_\theta \sum_{i=1}^N \norm{\pb[i] - r(\sB[i];\theta)} \label{eq:warmstart}
	\end{align}
	by solving a non-linear least squares problem, where the objective is to minimize the discrepancy between the estimated positions from binocular vision and the positions predicted by the reconstruction curve \( r(s[i];\theta) \). This optimization is carried out with known correspondences, offering a significant advantage in initializing our gradient descent process even though containing \mkh{noisy/faulty/inaccurate} data.
	
	By establishing this initial guess, we enable the subsequent iterative closest point algorithm to converge to a superior local minimum.


\subsection{Sectionname ist noch WIP -- Reconstruction function for easy sampling}
%Up until now, we considered arbitrary formulations for the reconstruction $r$.\ 
%As we want \mkh{needs to be clear why this is good} to be able to accurately sample the tube equidistantly, a fitting formulation for $r$ needs to be chosen.\ 
%For this, we lend from \CM \eqref{eq:CM_p}-\eqref{eq:CM_R0}, which describe an orthonormal frame moving through the euclidean space under rotations \mkh{not the nicest formulation...}.\
%In the following, our aim is to find the parameters of curvature functions $\boldu_n(s; \theta)$, such that the resulting curve 
%\begin{align*}
%	r(s, \boldu) &= \p(s)\\
%	{\p'}(s) &= \Rm(s)\bolde_3,\\
%	{\Rm'}(s) &= \Rm(s)\hat{\boldu}(s), \label{eq:CM_R}\\
%	\p(0) &= \p^0 \in \R^3\\
%	\Rm(0) &= \Rm^0 \in \SO
%\end{align*}
%\mkh{ich will damit ausdrücken, dass $r(s, \boldu)$ die Lösung der ODE darstellt.}
%While unconventional, this approach gives us an easy way of sampling with predefined-arclength and
%meets our goal of describing the image pixels.\
To this point, our discussion of the reconstruction curve \( r \) has been for general formulations.\
However, to effectively and accurately sample the continuum robot's structure, a specific mathematical representation for \( r \) is necessary.\
Our goal is to describe \( r \) in a way that enables equidistant sampling along its actual arc-length \( s \), not merely as a running variable, but as a true measure of the length along the curve.\

This can be achieved by adopting the rotating frame concept from differential geometry, specifically the same formulae as used by the CTCR model equations (referenced in \CM \eqref{eq:CM_p}-\eqref{eq:CM_R0}).\
This model describes the motion of an orthonormal frame in space under the influence of rotations, making it suitable for continuum robots.\
\figref{fig:frame} shows an exemplatory curve traced by a moving frame, where the curvatures \( \boldu = \begin{bmatrix}
	u_x & u_y & u_z
\end{bmatrix} \) rotate the frame around its axes.

We aim to determine the curvature function \( \boldu(s; \theta) \), where \( \theta \) are the decision variables influencing the curvature, resulting in a curve \( r(s, \theta) \).\ 
The curve is defined as the solution to the differential equation
\begin{align*}
	r(s, \theta) &= \p(s),\\
	\p'(s) &= \Rm(s)\bolde_3,\\
	\Rm'(s) &= \Rm(s)\boldu\hat{}(s; \theta),\\
	\p(0) &= \p^0 \in \R^3,\\
	\Rm(0) &= \Rm^0 \in \SO\\
	\text{with}\ \boldu\hat{} &= \begin{bmatrix}
		0 & -u_z & u_y \\
		u_z & 0 & -u_x \\
		-u_y & u_x & 0
	\end{bmatrix}.
\end{align*}
Here, \( \p(s) \) and \( \Rm(s) \) denote the position and orientation of the frame at any point along the arc-length \( s \).

This approach, albeit unconventional, offers a systematic and precise method for generating a curve with predefined arc-length sampling.
Moreover, the moving frame showed to be numerically more efficient than for example polynomials for the three coordinates of \( p(s) \).

\begin{figure}[htb]
	\centering
	\input{figs/moving_frame.tex}
	\caption{A 3D curve traced by a moving frame.\ 
		The frame follows its own z-axis and rotates around the axes with the curvatures $u_x$, $u_y$, and $u_z$.}
	\label{fig:frame}
\end{figure}




==> inc/Zusammenfassung.tex <==
% !TeX spellcheck = de_DE
% !TeX root = ..\main.tex

\setcounter{section}{-1}
\section{Zusammenfassung Rekonstruktionspaper}

Im Rahmen des SPP benötigen wir belastbare Daten über den Verlauf des Rückgrats der CTCRs, um Datenbasierte Modellverbesserungen vornehmen zu können. Die Rekonstruktion des Rückgrats stellt sich dabei als schwierig heraus, da die automatische Detektion von Rückgratpunkten über beispielsweise Interest Points aufgrund der einheitlichen Farbe nicht möglich ist und auch Markierungen sich als nicht hilfreich herausgestellt haben, da diese während der Aktuation verwischen. Aus diesem Grund stellen wir in diesem Paper einen auf Optimierungsverfahren basierenden Rekonstruktionsalgorithmus vor, der eine 3D-Kurve zu finden versucht, die die Daten eines Fotogrammetriesystems am besten beschreibt. Bei der Quellensuche sind wir auf ein ähnliches Verfahren basierend auf Differentiable Rendering (DR) \cite{lu2023diffrendering} gestoßen, bei dem ein vereinfachtes 3D-Volumen des Roboters gerendert (ein echtes 3D-Rendering wie es für Computer-generierte Grafiken verwendet wird) und dieses auf Bilddaten gefittet wird. Unser Algorithmus unterscheidet sich dreierlei von diesem Verfahren:
\begin{enumerate}
	\item Wir arbeiten rein mit dem Roboterrückgrat, wodurch keine Generierung des Volumens notwendig ist.
	\item Im DR Paper wird die Kostenfunktion als Summe aller Distanzen von Rekonstruktion zu Pixeln definiert, wir rechnen von Pixeln zu Rekonstruktion, da so der Algorithmus robuster wird (Figure sollte vmtl. im Paper noch ergänzt werden).
	\item Im DR Paper werden zusätzlich 4 Punkte entlang des Rückgrats rudimentär in die Bilder des Roboters gelegt und auf 4 Punkte entlang der Rekonstruktion gefittet, wir "lernen" die Zugehörigkeiten mittels eines Iterative Closest Point Algorithmus.
\end{enumerate}

Zunächst erklären wir Zhaohengs Algorithmus, der rein auf Bildverarbeitungs- und Computer Vision-Algorithmen basiert. \figref{fig:epipolar_geometry} zeigt die hierfür genutzte Epipolargeometrie. Diese besagt, dass der zu einem Pixel zugehörige 3-dimensionale Punkt in einem Bild 1 auf einer Linie in einem Bild 2 ebenfalls zu finden ist. Nach Reduktion der Kanülen auf Linien (mittels Skelettierung) können so mehrere 3D-Punkte gefunden werden. Die Position entlang des Rückgrats kann nicht kontrolliert werden, wenn Fehler in der Kameramatrix vorhanden sind, was zu Verschiebungen in den Projektionslinien führen kann, insbesondere an den Wendepunkten der 3D-Kurve. Und es fehlen zudem exakte Informationen über die Bogenlänge eines Punktes, allerdings kann diese über kumulativ aufsummierte Distanzen abgeschätzt werden. Dieser Algorithmus eignet sich sehr gut, um den optimierungsbasierten Algorithmus warmzustarten.

Numerische Ergebnisse folgen noch.

Kapitel 6 leitet daraufhin den optimierungsbasierten Algorithmus. Wir starten mit dem allgemeinen Minimierungsproblem um die Abweichung zweier kontinuierlicher Kurven \( b \) -- das auf den Bildern aufgezeichnete Rückgrat -- und \( r \) -- die Rekonstruktion als 3D-Kurve -- zu minimieren und treffen daraufhin Einschränkungen, die wir aufgrund unseres Settings haben. Speziell sind diese
\begin{enumerate}
	\item Wir kennen die Funktion von \( b \) nicht und sehen von \( b \) auch nur Projektionen.
	\item Von den Projektionen von \( b \) kennen wir darüber hinaus auch nur diskrete Punkte (Pixel) \( b(\sbi) \).
	\item Wir kennen die Werte von $\sbi$ nicht, können also kein direktes Matching betreiben.
\end{enumerate}

Daraufhin formuliere ich das Optimierungsproblem als Bi-Level-Optimierungsproblem, in dem wir auf dem oberen Leven die Abweichung zueinander gehöriger Punkte minimieren, auf einem unteren Level aber die Zugehörigkeit bestimmen. 
Durch Entkopplung dieser Optimierungsprobleme erhält man dann einen Iterative Closest Point Algorithmus.
Von diesem lässt sich zeigen, dass er immer zu lokalen Lösungen konvergiert. Mithilfe dieses Beweises leite ich zwei Algorithmen ab, den \ms Algorithmus, der sich aus den bisherigen Betrachtungen ergibt, und die \os Formulierung, die im Gegensatz nach jedem Matching von Punkten nur einen einzelnen Gradientenabstiegsschritt vollführt.

Die nächste Subsection erklärt, dass gradienten-basierte Verfahren zu lokalen Minima laufen und dass ein guter initial guess (wie bspw. durch Zhaohengs Algorithmus) die Ergbenisse verbessern kann.

Subsection 6.3 erklärt danach wie wir \( r \) parametrieren, nämlich als moving frame, wie es im zweiten Teil des Rucker-Modells geschieht. Das passt einerseits zu den von uns betrachteten Robotern und ist numerisch (aus einem mir nicht ganz schlüssigen Grund) effizienter als bspw. drei Polynome.

Die numerischen Ergebnisse des Optimierungsbasierten Ansatzes zeigen, dass ohne Warmstarting die \os Formulierung zufriedenstellende Ergebnisse liefert, die \ms Formulierung in ein lokales Minimum läuft. Daraufhin wird mit Warmstarting gezeigt, dass beide zu guten Ergebnissen konvergieren, die \os Formulierung aber überlegen ist.

==> inc/todo.tex <==
% !TeX spellcheck = en_US
% !TeX root = ..\main.tex

\section{General ToDos}

\begin{itemize}
	\item Discussion about \enquote{camera calibration} vs. \enquote{camera (parameter) identification}
\end{itemize}
